Unstructured Evidence Attribution for Long Context Query Focused Summarization

Large language models (LLMs) are capable of generating coherent summaries from very long contexts given a user query, and extracting and citing evidence spans helps improve the trustworthiness of these summaries. Whereas previous work has focused on evidence citation with fixed levels of granularity (e.g. sentence, paragraph, document, etc.), we propose to extract unstructured (i.e., spans of any length) evidence in order to acquire more relevant and consistent evidence than in the fixed granularity case. We show how existing systems struggle to copy and properly cite unstructured evidence, which also tends to be "lost-in-the-middle". To help models perform this task, we create the Summaries with Unstructured Evidence Text dataset (SUnsET), a synthetic dataset generated using a novel pipeline, which can be used as training supervision for unstructured evidence summarization. We demonstrate across 5 LLMs and 4 datasets spanning human written, synthetic, single, and multi-document settings that LLMs adapted with SUnsET generate more relevant and factually consistent evidence with their summaries, extract evidence from more diverse locations in their context, and can generate more relevant and consistent summaries than baselines with no fine-tuning and fixed granularity evidence. We release SUnsET and our generation code to the public.

==> abstractive_results.tex <==

\begin{table}%
    \def\arraystretch{1.2}
    \centering
    \scriptsize
    
    \begin{tabular}{l c c | c c | c c | c c}
    \toprule %
    & \multicolumn{2}{ c |}{ Squality } & \multicolumn{2}{c|}{ LexAbSumm } & \multicolumn{2}{c |}{ SummHay } & \multicolumn{2}{c}{ ScholarQABench }\\
    \midrule
    Method & Rel & Con & Rel & Con & Rel & Con & Rel & Con\\

\midrule
Base &  2.75 & 2.21 & \textbf{3.71} & \textbf{3.34} & 4.62 & 4.51 & 3.82 & 3.64 \\
~~~+ Standard & \textbf{2.86}** & \textbf{2.28}** & 3.35 & 3.05 & 4.58 & 4.47 & 3.80 & 3.59 \\
~~~+ Shuffled & 2.68 & 2.14 & 3.50 & 3.17 & \textbf{4.67} & \textbf{4.56} & \textbf{3.92}** & \textbf{3.68} \\
~~~+ Fused & 2.68 & 2.11 & 3.38 & 3.09 & - & - & - & - \\
Base &  \textbf{4.39} & \textbf{4.07} & - & - & 4.75 & 4.71 & 4.30 & 4.11 \\
~~~+ Standard & 4.13 & 3.71 & 4.21 & \textbf{4.03} & 4.90** & 4.83** & 4.44** & \textbf{4.21}** \\
~~~+ Shuffled & 3.80 & 3.39 & \textbf{4.28} & 4.01 & \textbf{4.93}** & \textbf{4.85}** & 4.40** & 4.14 \\
~~~+ Fused & 4.12 & 3.63 & 4.16 & 3.98 & 4.91** & 4.83** & \textbf{4.46}** & 4.17** \\
    \bottomrule %

    \end{tabular}
    \caption{Relevance and consistency of generated summaries. Relevance and consistency are measured using an autorater (GPT-4o-mini)~\cn{} based on previously validated prompts~\cn{}. ** indicates significance as measured by non-overlapping bootstrapped confidence intervals with the baseline.}
    \label{tab:retrieval_results}
\end{table}


==> figures/performance_vs_data.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{latex/figures/variable_data/llama_3.2_1B_RC_plot_squality.pdf}
    \vspace{1pt}
    \caption{Llama 3.2 1B}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=1\linewidth]{latex/figures/variable_data/llama_3.1_8B_RC_plot_squality.pdf}
    \vspace{1pt}
        
    \caption{Llama 3.1 8B}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=1 \linewidth]{latex/figures/variable_data/mixtral_8x7B_RC_plot_squality.pdf}
    \vspace{1pt}
        
    \caption{Mixtral 8x7B}
    \end{subfigure}
    ~%
        
        
\caption{SQuALITY: Relevance and consistency performance vs. number of synthetic training samples.}
        \label{fig:variable_data_squality}
\end{figure*}%

\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{latex/figures/variable_data/llama_3.2_1B_RC_plot_scholarQA.pdf}
    \vspace{1pt}
    
    \caption{Llama 3.2 1B}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=1\linewidth]{latex/figures/variable_data/llama_3.1_8B_RC_plot_scholarQA.pdf}
    \vspace{1pt}
    
    \caption{Llama 3.1 8B}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=1\linewidth]{latex/figures/variable_data/mixtral_8x7B_RC_plot_scholarQA.pdf}
    \vspace{1pt}
    
        \caption{Mixtral 8x7B}
    \end{subfigure}
    
    
\caption{ScholarQABench: Relevance and consistency performance vs. number of synthetic training samples.}
        \label{fig:variable_data_ScholarQABench}
\end{figure*}%


==> figures/positional_bias_figures.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/meta-llama_Llama-3.2-1B-Instruct_locations_alt.pdf}
    \caption{Llama 3.2 1B}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/meta-llama_Llama-3.2-3B-Instruct_locations_alt.pdf}
    \caption{Llama 3.2 3B}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/meta-llama_Meta-Llama-3.1-8B-Instruct_locations_alt.pdf}
        \caption{Llama 3.1 8B}
    \end{subfigure}
    \\
    \vspace{-3pt}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/mistralai_Mistral-Nemo-Instruct-2407_locations_alt.pdf}
        \caption{Mistral Nemo 2407}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/mistralai_Mixtral-8x7B-Instruct-v0.1_locations_alt.pdf}
        \caption{Mixtral 8x7B}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/gpt-4o-mini_locations_alt.pdf}
        \caption{GPT 4o Mini}
    \end{subfigure}
    
\caption{Location of extracted evidence in the provided source context for different methods.}
\label{fig:evidence_location}
\end{figure*}%
    
        
        
        


==> figures/positional_bias_figures_alt.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.27\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/meta-llama_Llama-3.2-3B-Instruct_locations_alt.pdf}
    \caption{Llama 3.2 3B}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.27\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/meta-llama_Meta-Llama-3.1-8B-Instruct_locations_alt.pdf}
        \caption{Llama 3.1 8B}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.27\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/gpt-4o-mini_locations_alt.pdf}
        \caption{GPT 4o Mini}
    \end{subfigure}
    \\
    \vspace{-3pt}
    \begin{subfigure}[t]{0.27\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/mistralai_Mistral-Nemo-Instruct-2407_locations_alt.pdf}
        \caption{Mistral Nemo 2407}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.27\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/mistralai_Mixtral-8x7B-Instruct-v0.1_locations_alt.pdf}
        \caption{Mixtral 8x7B}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.27\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/combined_ground_truth.pdf}
        \caption{Test Datasets}
    \end{subfigure}
    
\caption{Distribution of location of extracted evidence in the provided source context for different methods. Test dataset evidence location is measured by comparing to reference summaries.}
\label{fig:evidence_location}
\end{figure*}%
    
        
        
        


==> latex/figures/positional_bias_figures.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/meta-llama_Llama-3.2-1B-Instruct_locations_alt.pdf}
    \caption{Llama 3.2 1B}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/meta-llama_Llama-3.2-3B-Instruct_locations_alt.pdf}
    \caption{Llama 3.2 3B}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/meta-llama_Meta-Llama-3.1-8B-Instruct_locations_alt.pdf}
        \caption{Llama 3.1 8B}
    \end{subfigure}
    \\
    \vspace{-3pt}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/mistralai_Mistral-Nemo-Instruct-2407_locations_alt.pdf}
        \caption{Mistral Nemo 2407}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/mistralai_Mixtral-8x7B-Instruct-v0.1_locations_alt.pdf}
        \caption{Mixtral 8x7B}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.32\textwidth}
        \centering\includegraphics[width=0.88\linewidth]{latex/figures/evidence_locations/gpt-4o-mini_locations_alt.pdf}
        \caption{GPT 4o Mini}
    \end{subfigure}
    
\caption{Location of extracted evidence in the provided source context for different methods.}
\label{fig:evidence_location}
\end{figure*}%
% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[t]{0.23\textwidth}
%     \centering
%     \includegraphics[width=0.98\linewidth]{latex/figures/gt_evidence/pszemraj_SQuALITY-v1.3_evidence_dist.pdf}
    
%     \caption{\sqa{}}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.23\textwidth}
%         \centering\includegraphics[width=0.98\linewidth]{latex/figures/gt_evidence/MahmoudAly_LexAbSumm_evidence_dist.pdf}
        
%     \caption{\las{}}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.23\textwidth}
%         \centering\includegraphics[width=0.98\linewidth]{latex/figures/gt_evidence/Salesforce_summary-of-a-haystack_evidence_dist.pdf}
        
%     \caption{\smh{}}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.23\textwidth}
%         \centering\includegraphics[width=0.98\linewidth]{latex/figures/gt_evidence/data_ScholarQABench__evidence_dist.pdf}
        
%     \caption{\ops{}}
%     \end{subfigure}
% \caption{Location of ground truth evidence in each dataset.}
% \label{fig:gt_distribution}
% \end{figure*}%

==> latex/tables/GPT-J_results.tex <==

\begin{table}%[htp]
    %\setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.2}
    \centering
    %\fontsize{10}{10}\selectfont
    \scriptsize
    %\rowcolors{2}{gray!10}{white}
    \begin{tabular}{l c c c c}
    \toprule %\thickhline
    Method & Coherence & Relevance & Faithfulness & ...\\

\midrule

    \bottomrule % \thickhline

    \end{tabular}
    \caption{Results when using GPT-J to simulate human judgments.} %Results are reported as the average macro F1 over 5 random seeds.}
    \label{tab:abstractive_results}
\end{table}


==> latex/tables/abstractive_results_original.tex <==

\begin{table}[t]
    \setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.1}
    \centering
    %\fontsize{10}{10}\selectfont
    \scriptsize
    %\rowcolors{2}{gray!10}{white}
    
    \begin{tabular}{l c c | c c | c c | c c}
    \toprule %\thickhline
    & \multicolumn{2}{ c |}{ SLT\textsuperscript{S} } & \multicolumn{2}{c|}{ LAS\textsuperscript{S} } & \multicolumn{2}{c |}{ SMH\textsuperscript{M} } & \multicolumn{2}{c}{ SQB\textsuperscript{M} }\\
    \midrule
    Method & Rel & Con & Rel & Con & Rel & Con & Rel & Con\\

\midrule
Llama 3.2 1B & 2.68 & 2.15 & \textbf{3.68} & \textbf{3.38} & 4.53 & 4.40 & 3.80 & 3.61 \\
~~~+ Standard & 2.73\textsuperscript{=} & \textbf{2.17}\textsuperscript{=} & 3.25 & 2.93 & 4.53\textsuperscript{=} & 4.44\textsuperscript{=} & 3.81\textsuperscript{=} & 3.59\textsuperscript{=} \\
~~~+ Shuffled & \textbf{2.79}* & 2.15\textsuperscript{=} & 3.41 & 3.03 & \textbf{4.66}* & \textbf{4.55}* & \textbf{3.97}* & \textbf{3.69}* \\\midrule
Llama 3.2 3B & \textbf{4.39} & \textbf{4.05} & \textbf{4.40} & \textbf{4.19} & 4.82 & 4.74 & 4.28 & 4.11 \\
~~~+ Standard & 4.22 & 3.80 & 4.19 & 4.02 & \textbf{4.90}* & \textbf{4.85}* & 4.41* & 4.21* \\
~~~+ Shuffled & 3.84 & 3.38 & 4.25 & 4.02 & 4.89* & 4.84* & \textbf{4.49}* & \textbf{4.23}* \\\midrule
Llama 3.1 8B & 4.55 & 4.34 & \textbf{4.64} & \textbf{4.52} & 4.88 & 4.78 & 4.18 & 4.06 \\
~~~+ Standard & \textbf{4.63}* & \textbf{4.41}* & 4.53 & 4.44 & 4.94* & \textbf{4.93}* & 4.64* & \textbf{4.42}* \\
~~~+ Shuffled & 4.59* & 4.34\textsuperscript{=} & 4.55 & 4.44 & \textbf{4.97}* & 4.92* & \textbf{4.68}* & 4.41* \\\midrule
Mistral Nemo 2407 & 4.27 & 4.09 & 3.83 & 3.85 & 4.27 & 4.15 & 3.15 & 3.23 \\
~~~+ Standard & 4.43* & 4.24* & 4.03* & 4.04* & 4.54* & 4.47* & \textbf{3.79}* & \textbf{3.75}* \\
~~~+ Shuffled & \textbf{4.53}* & \textbf{4.35}* & \textbf{4.18}* & \textbf{4.12}* & \textbf{4.65}* & \textbf{4.49}* & 3.49* & 3.41* \\\midrule
Mixtral 8x7B & 4.02 & 3.99 & 4.28 & 4.22 & 4.78 & 4.68 & 3.95 & 3.89 \\
~~~+ Standard & \textbf{4.52}* & 4.35* & \textbf{4.45}* & \textbf{4.40}* & \textbf{4.84}* & \textbf{4.72}* & 4.26* & 4.13* \\
~~~+ Shuffled & 4.51* & \textbf{4.40}* & 4.44* & 4.38* & 4.79\textsuperscript{=} & 4.68\textsuperscript{=} & \textbf{4.33}* & \textbf{4.18}* \\\midrule
\midrule
GPT 4o Mini & \textit{4.98} & \textit{4.92} & \textit{4.93} & \textit{4.77} & \textit{4.99} & \textit{4.98} & \textit{4.94} & \textit{4.76} \\
    \bottomrule % \thickhline

    \end{tabular}
    \caption{Relevance and consistency of generated summaries. Relevance and consistency are measured using an autorater (GPT-4o-mini,~\citet{DBLP:conf/emnlp/LiuIXWXZ23}) based on previously validated prompts~\cite{DBLP:journals/corr/abs-2410-23463}. 
    * indicates significance as measured by non-overlapping bootstrapped confidence intervals with the baseline. \textsuperscript{=} indicates no significant difference from baseline.
    \textsuperscript{S} indicates single document tasks, \textsuperscript{M} indicates multi-document. SLT is \sqa{}, LAS is \las{}, SH is \smh{}, and SQB is \ops{}.}
    \vspace{-10pt}
    \label{tab:abstractive_results}
\end{table}


==> latex/tables/citation_results.tex <==

\begin{table*}[t]
    %\setlength{\tabcolsep}{1.5pt}
    %\def\arraystretch{1.1}
    \centering
    %\fontsize{9}{9}\selectfont
    %\scriptsize
    %\rowcolors{2}{gray!10}{white}

    \begin{tabular}{l c c | c c | c c | c c}
    \toprule %\thickhline
    & \multicolumn{2}{ c |}{ SLT\textsuperscript{S} } & \multicolumn{2}{c|}{ LAS\textsuperscript{S} } & \multicolumn{2}{c |}{ SMH\textsuperscript{M} } & \multicolumn{2}{c}{ SQB\textsuperscript{M} }\\
    \midrule
    Model & Rel\textsubscript{F1} & Con\textsubscript{F1} & Rel\textsubscript{F1} & Con\textsubscript{F1} & Rel\textsubscript{F1} & Con\textsubscript{F1} & Rel\textsubscript{F1} & Con\textsubscript{F1}\\

\midrule
Llama 3.2 1B &  $0.14$ & $0.14$ & $1.22$ & $0.84$ & $0.36$ & $0.00$ & $0.11$ & $0.14$ \\
Fixed Gran. & $0.40$ & $0.13$ & $\underline{6.67}$ & $\underline{4.40}$ & $\underline{0.39}$ & $\underline{0.19}$ & $2.27$ & $\underline{1.35}$ \\
+ SUnsET & $1.18$ & $0.62$ & $5.43$ & $3.59$ & $0.00$ & $0.00$ & $\underline{3.13}$ & $1.26$ \\
+ Shuffled & $\underline{1.85}$ & $\underline{0.80}$ & $3.14$ & $3.04$ & $0.08$ & $0.00$ & $0.85$ & $0.72$ \\\midrule
Llama 3.2 3B &  $6.61$ & $3.86$ & $15.17$ & $13.29$ & $7.66$ & $6.52$ & $14.12$ & $10.54$ \\
Fixed Gran. & $21.71$ & $9.02$ & $\underline{45.80}$ & $\underline{41.44}$ & $1.37$ & $1.13$ & $\underline{27.77}$ & $\underline{23.49}$ \\
+ SUnsET & $\underline{25.36}$ & $\underline{14.76}$ & $33.42$ & $29.40$ & $\underline{32.21}$ & $\underline{29.59}$ & $13.76$ & $11.85$ \\
+ Shuffled & $15.14$ & $9.33$ & $19.45$ & $16.80$ & $26.78$ & $25.15$ & $17.45$ & $16.55$ \\\midrule
Llama 3.1 8B &  $11.66$ & $7.38$ & $28.89$ & $26.76$ & $32.07$ & $29.17$ & $20.73$ & $16.32$ \\
Fixed Gran. & $18.90$ & $11.32$ & $42.44$ & $38.86$ & $14.29$ & $14.23$ & $38.56$ & $37.64$ \\
+ SUnsET & $\underline{27.69}$ & $\underline{18.48}$ & $\mathbf{\underline{\mathbf{50.78}}}$ & $\mathbf{\underline{\mathbf{47.62}}}$ & $\mathbf{\underline{\mathbf{53.62}}}$ & $\mathbf{\underline{\mathbf{51.43}}}$ & $\mathbf{\underline{\mathbf{44.03}}}$ & $\underline{40.49}$ \\
+ Shuffled & $23.13$ & $16.12$ & $44.16$ & $41.18$ & $48.72$ & $46.50$ & $41.49$ & $39.59$ \\\midrule
Mistral Nemo 2407 &  $0.53$ & $0.23$ & $1.36$ & $1.29$ & $6.68$ & $6.68$ & $6.08$ & $5.54$ \\
Fixed Gran. & $6.61$ & $3.93$ & $13.36$ & $11.95$ & $3.71$ & $3.36$ & $15.05$ & $11.03$ \\
+ SUnsET & $\underline{21.71}$ & $\underline{13.99}$ & $\underline{23.38}$ & $\underline{23.09}$ & $\underline{20.73}$ & $\underline{19.71}$ & $\underline{22.00}$ & $\underline{20.61}$ \\
+ Shuffled & $17.67$ & $11.96$ & $22.85$ & $22.42$ & $19.82$ & $18.38$ & $16.87$ & $16.14$ \\\midrule
Mixtral 8x7B &  $17.83$ & $12.64$ & $34.27$ & $35.23$ & $33.40$ & $32.02$ & $17.30$ & $15.48$ \\
Fixed Gran. & $\mathbf{\underline{\mathbf{36.35}}}$ & $\mathbf{\underline{\mathbf{20.33}}}$ & $\underline{42.34}$ & $\underline{40.15}$ & $8.45$ & $7.46$ & $\underline{40.06}$ & $\mathbf{\underline{\mathbf{44.4}0}}$ \\
+ SUnsET & $22.60$ & $16.11$ & $35.81$ & $35.81$ & $42.91$ & $42.27$ & $28.61$ & $26.94$ \\
+ Shuffled & $23.79$ & $17.85$ & $37.21$ & $37.57$ & $\underline{43.89}$ & $\underline{42.98}$ & $32.25$ & $31.16$ \\\midrule
\midrule GPT 4o Mini &  \textit{37.39} & \textit{31.70} & \textit{61.17} & \textit{58.68} & \textit{63.61} & \textit{62.35} & \textit{33.71} & \textit{28.63} \\
    \bottomrule % \thickhline

    \end{tabular}
    \caption{Relevance and consistency of evidence sentences with respect to their citances. Relevance and consistency are measured using an autorater (DeepSeek-V3)~\cite{DBLP:conf/emnlp/LiuIXWXZ23} based on previously validated prompts~\cite{DBLP:journals/corr/abs-2410-23463}. 
    We follow a similar setup to \cite{DBLP:conf/emnlp/LabanFXW24,openscholar} where we measure citation precision and recall in order to calculate an overall F1 score for both relevance and consistency. 
    \	extbf{Bold} indicates best overall performance, \underline{Underline} indicates best performance for individual models.
    \textsuperscript{S} indicates single document tasks, \textsuperscript{M} indicates multi-document. SQ is \sqa{}, LAS is \las{}, SMH is \smh{}, and SQB is \ops{}}
    \label{tab:retrieval_results}
\end{table*}


==> latex/tables/citation_results_original.tex <==

\begin{table}[t]
    \setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.1}
    \centering
    %\fontsize{10}{10}\selectfont
    \scriptsize
    %\rowcolors{2}{gray!10}{white}

    \begin{tabular}{l c c | c c | c c | c c}
    \toprule %\thickhline
    & \multicolumn{2}{ c |}{ SLT\textsuperscript{S} } & \multicolumn{2}{c|}{ LAS\textsuperscript{S} } & \multicolumn{2}{c |}{ SMH\textsuperscript{M} } & \multicolumn{2}{c}{ SQB\textsuperscript{M} }\\
    \midrule
    Method & Rel\textsubscript{F1} & Con\textsubscript{F1} & Rel\textsubscript{F1} & Con\textsubscript{F1} & Rel\textsubscript{F1} & Con\textsubscript{F1} & Rel\textsubscript{F1} & Con\textsubscript{F1}\\

\midrule
Llama 3.2 1B &  0.00 & 0.00 & 0.94 & 1.06 & \textbf{0.00} & \textbf{0.00} & 0.23 & 0.18 \\
~~~+ Standard & \textbf{0.63} & \textbf{0.53} & \textbf{4.80} & \textbf{4.56} & \textbf{0.00} & \textbf{0.00} & \textbf{1.84} & \textbf{1.68} \\
~~~+ Shuffled & 0.48 & 0.26 & 2.83 & 2.84 & \textbf{0.00} & \textbf{0.00} & 0.00 & 0.00 \\\midrule
Llama 3.2 3B &  11.21 & 10.16 & 15.08 & 14.64 & 8.64 & 8.75 & 12.37 & 12.99 \\
~~~+ Standard & \textbf{36.19} & \textbf{25.12} & \textbf{43.98} & \textbf{40.64} & \textbf{37.73} & \textbf{39.03} & \textbf{37.16} & \textbf{34.39} \\
~~~+ Shuffled & 23.38 & 15.33 & 36.19 & 31.26 & 32.73 & 33.46 & 31.36 & 26.73 \\\midrule
Llama 3.1 8B &  17.21 & 15.15 & 31.17 & 30.65 & 34.18 & 37.96 & 32.08 & 32.85 \\
~~~+ Standard & \textbf{35.21} & \textbf{25.34} & \textbf{52.64} & \textbf{47.79} & \textbf{56.82} & \textbf{57.50} & \textbf{45.26} & \textbf{41.13} \\
~~~+ Shuffled & 29.36 & 20.65 & 49.90 & 44.19 & 54.79 & 54.27 & 39.53 & 36.17 \\\midrule
Mistral Nemo 2407 &  2.75 & 2.37 & 5.34 & 4.58 & 10.37 & 10.25 & 5.67 & 5.36 \\
~~~+ Standard & \textbf{34.24} & \textbf{24.45} & 38.21 & 36.88 & \textbf{23.54} & \textbf{25.13} & \textbf{7.15} & \textbf{7.56} \\
~~~+ Shuffled & 32.52 & 22.84 & \textbf{39.94} & \textbf{38.57} & 21.58 & 23.23 & 4.65 & 4.08 \\\midrule
Mixtral 8x7B &  24.45 & 19.15 & 39.48 & 40.08 & 44.01 & 43.44 & 25.97 & 25.61 \\
~~~+ Standard & 30.54 & 25.11 & 38.27 & 38.08 & \textbf{48.71} & \textbf{51.85} & 38.37 & 38.59 \\
~~~+ Shuffled & \textbf{32.87} & \textbf{25.86} & \textbf{44.13} & \textbf{44.48} & 46.67 & 49.09 & \textbf{39.65} & \textbf{41.89} \\\midrule
\midrule GPT 4o Mini &  \textit{42.62} & \textit{36.23} & \textit{59.48} & \textit{53.96} & \textit{64.99} & \textit{60.14} & \textit{37.65} & \textit{33.11} \\
    \bottomrule % \thickhline

    \end{tabular}
    \caption{Relevance and consistency of evidence sentences with respect to their citances. Relevance and consistency are measured using an autorater (GPT-4o-mini)~\cite{DBLP:conf/emnlp/LiuIXWXZ23} based on previously validated prompts~\cite{DBLP:journals/corr/abs-2410-23463}. 
    We follow a similar setup to \cite{DBLP:conf/emnlp/LabanFXW24,openscholar} where we measure citation precision and recall in order to calculate an overall F1 score for both relevance and consistency. 
    \textsuperscript{S} indicates single document tasks, \textsuperscript{M} indicates multi-document. SQ is \sqa{}, LAS is \las{}, SMH is \smh{}, and SQB is \ops{}}
    \label{tab:retrieval_results}
\end{table}


==> latex/tables/results_evidence_loading.tex <==

\begin{table*}[t]
    %\setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.2}
    \centering
    %\fontsize{10}{10}\selectfont
    \scriptsize
    %\rowcolors{2}{gray!10}{white}

    \begin{tabular}{l | c c | c c}
    \toprule %\thickhline
    &  \multicolumn{2}{c |}{ SummHay\textsuperscript{M} } & \multicolumn{2}{c}{ ScholarQABench\textsuperscript{M} }\\
    \midrule
    Method &  Rel & Con & Rel & Con\\

\midrule
Llama 3.1 8B &  4.86 & 4.78 & 4.23 & 4.07 \\
~~~Basline Front Loading & 4.86\textsuperscript{=} & 4.81\textsuperscript{=} & 4.23\textsuperscript{=} & 4.05\textsuperscript{=} \\
~~~Basline Back Loading & 4.87\textsuperscript{=} & 4.82* & 4.18 & 4.02 \\
Trained & \textbf{4.96}* & 4.91* & \textbf{4.64}* & \textbf{4.40}* \\
~~~Trained Front Loading & 4.95* & \textbf{4.92}* & 4.58* & 4.36* \\
~~~Trained Back Loading & 4.95* & 4.90* & 4.61* & 4.39* \\
    \bottomrule % \thickhline

    \end{tabular}
    \caption{Relevance and consistency of generated summaries. Relevance and consistency are measured using an autorater (GPT-4o-mini)~\cn{} based on previously validated prompts~\cn{}. 
    * indicates significance as measured by non-overlapping bootstrapped confidence intervals with the baseline. \textsuperscript{=} indicates no significant difference from baseline.
    \textsuperscript{S} indicates single document tasks, \textsuperscript{M} indicates multi-document.}
    \label{tab:retrieval_results}
\end{table*}


==> latex/tables/synthetic_data_backup.tex <==

\begin{table*}%[htp]
    \setlength{\tabcolsep}{2pt}
    \def\arraystretch{1.1}
    \centering
    %\scalebox{0.8}{
    %\fontsize{10}{10}\selectfont
    \scriptsize
    %\rowcolors{2}{gray!10}{white}
    \begin{tabular}{r c c c c | c c c c | c c c c}
    \toprule %\thickhline
    & \multicolumn{4}{ c |}{ \dataset{} } & \multicolumn{4}{c|}{ Base } & \multicolumn{4}{c}{ Base w/ Titles  } \\
    \midrule
    
    Method & Titles & Questions & Summaries & Documents & Titles & Questions & Summaries & Documents & Titles & Questions & Summaries & Documents \\
    %TTR & 0.584 & 0.188 & 0.067 & 0.036 & 0.123 & 0.123 & 0.143 & 0.000 & 0.261 & 0.105 & 0.113 & 0.000 \\
    %Root TTR & 13.64 & 15.19 & 22.58 & 21.96 & 3.20 & 8.68 & 15.51 & 0.098 & 6.26 & 7.50 & 12.49 & 0.103 \\
    %Log TTR & 0.915 & 0.810 & 0.768 & 0.741 & 0.678 & 0.754 & 0.792 & 0.313 & 0.790 & 0.736 & 0.768 & 0.316 \\
    %Maas TTR & 0.031 & 0.050 & 0.050 & 0.050 & 0.114 & 0.067 & 0.051 & 0.127 & 0.077 & 0.071 & 0.057 & 0.128 \\
    Moving Avg. TTR & 0.816 & 0.751 & 0.836 & 0.820 & 0.387 & 0.670 & 0.797 & 0.350 & 0.588 & 0.631 & 0.778 & 0.352 \\
    Avg. Cosinse Dist. & 0.780 & 0.806 & 0.733 & 0.682 & 0.425 & 0.725 & 0.716 & 0.042 & 0.607 & 0.660 & 0.610 & 0.040 \\
    Avg. Length (in words) & 5.44 & 13.45 & 226.5 & 3767.4 & 6.65 & 9.85 & 23.79 & 474.8 & 5.76 & 10.21 & 24.45 & 433.8 \\
    
    
%\midrule

    \bottomrule % \thickhline

    \end{tabular}
    %}
    \caption{Statistics and diversity metrics of synthetically generated data.} %Results are reported as the average macro F1 over 5 random seeds.}
    \label{tab:synthetic_stats}
\end{table*}


==> latex/tables/table1.tex <==

\begin{table*}%[htp]
    %\setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.2}
    \centering
    %\fontsize{10}{10}\selectfont
    \scriptsize
    %\rowcolors{2}{gray!10}{white}
    \begin{tabular}{l c c c c}
    \toprule %\thickhline
    Method & R1 & R2 & RL & BERTScore\\

\midrule
\multicolumn{5}{c}{ACLSum \cite{DBLP:journals/corr/abs-2403-05303}}\\
\midrule
Llama2\textsubscript{ZS} \cite{DBLP:journals/corr/abs-2403-05303} & $26.17$&$9.43$&$18.91$&$64.00$ \\
Mistral\textsubscript{ZS}&$34.40$& $12.07$& $25.13$& $66.97$\\
Mistral\textsubscript{WiM}&$-$& $-$& $-$& $-$\\
Mistral\textsubscript{CB}&$33.75$& $11.73$& $24.69$& $66.59$\\
Mistral\textsubscript{CB-D}&$\mathbf{35.10}$& $12.44$& $25.12$& $\mathbf{67.63}$\\
Mistral\textsubscript{CB-FTD}&$34.67$& $12.29$& $\mathbf{25.58}$& $67.46$\\
Mistral\textsubscript{SB}&$33.41$& $11.13$& $24.24$& $66.45$\\
Mistral\textsubscript{SB-D}&$34.36$& $12.28$& $25.13$& $66.95$\\
Mistral\textsubscript{SB-FTD}&$33.95$& $11.77$& $24.71$& $66.96$\\
Llama3\textsubscript{ZS}&$33.85$& $12.61$& $24.74$& $67.09$\\
Llama3\textsubscript{WiM}&$32.70$& $12.91$& $24.79$& $66.18$\\
Llama3\textsubscript{CB}&$32.42$& $11.45$& $23.70$& $66.34$\\
Llama3\textsubscript{CB-D}&$34.03$& $12.28$& $24.87$& $67.23$\\
Llama3\textsubscript{CB-FTD}&$34.51$& $\mathbf{13.00}$& $25.04$& $67.33$\\
Llama3\textsubscript{SB}&$31.95$& $11.27$& $23.49$& $66.15$\\
Llama3\textsubscript{SB-D}&$33.54$& $12.61$& $24.71$& $66.84$\\
Llama3\textsubscript{SB-FTD}&$33.41$& $12.44$& $24.68$& $67.00$\\
\midrule
\multicolumn{5}{c}{SQuALITY \cite{DBLP:conf/emnlp/WangPCPB22}}\\
\midrule
BART+DPR \cite{DBLP:conf/emnlp/WangPCPB22} & $41.50$&$11.40$&$21.00$&$85.50$ \\
Mistral\textsubscript{ZS}&$\mathbf{37.75}$& $9.22$& $\mathbf{19.89}$& $\mathbf{61.48}$\\
Mistral\textsubscript{WiM}&$36.50$& $\mathbf{9.36}$& $19.34$& $59.01$\\
Mistral\textsubscript{CB}&$37.29$& $8.95$& $19.35$& $60.34$\\
Mistral\textsubscript{CB-D}&$36.92$& $8.54$& $19.29$& $60.73$\\
Mistral\textsubscript{CB-FTD}&$36.87$& $8.96$& $19.18$& $60.26$\\
Mistral\textsubscript{SB}&$-$& $-$& $-$& $-$\\
Mistral\textsubscript{SB-D}&$-$& $-$& $-$& $-$\\
Mistral\textsubscript{SB-FTD}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{ZS}&$34.18$& $8.26$& $18.11$& $55.47$\\
Llama3\textsubscript{WiM}&$33.34$& $8.78$& $18.12$& $57.25$\\
Llama3\textsubscript{CB}&$34.60$& $8.37$& $18.31$& $56.27$\\
Llama3\textsubscript{CB-D}&$34.57$& $8.20$& $18.28$& $56.07$\\
Llama3\textsubscript{CB-FTD}&$34.30$& $8.10$& $18.22$& $56.06$\\
Llama3\textsubscript{SB}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{SB-D}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{SB-FTD}&$-$& $-$& $-$& $-$\\
\midrule
\multicolumn{5}{c}{LexAbSumm \cite{DBLP:conf/coling/SantoshAG24}}\\
\midrule
Unlimiformer-BART \cite{DBLP:conf/coling/SantoshAG24} & $50.62$&$30.28$&$35.55$&$88.86$ \\
Mistral\textsubscript{ZS}&$36.97$& $14.54$& $20.07$& $59.64$\\
Mistral\textsubscript{WiM}&$34.91$& $13.26$& $19.26$& $57.97$\\
Mistral\textsubscript{CB}&$37.00$& $13.85$& $20.22$& $59.41$\\
Mistral\textsubscript{CB-D}&$37.80$& $14.83$& $20.57$& $59.93$\\
Mistral\textsubscript{CB-FTD}&$38.41$& $\mathbf{15.26}$& $20.79$& $\mathbf{60.36}$\\
Mistral\textsubscript{SB}&$-$& $-$& $-$& $-$\\
Mistral\textsubscript{SB-D}&$-$& $-$& $-$& $-$\\
Mistral\textsubscript{SB-FTD}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{ZS}&$\mathbf{39.47}$& $15.06$& $\mathbf{22.28}$& $59.43$\\
Llama3\textsubscript{WiM}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{CB}&$38.44$& $13.86$& $21.62$& $59.08$\\
Llama3\textsubscript{CB-D}&$38.77$& $14.64$& $21.81$& $59.33$\\
Llama3\textsubscript{CB-FTD}&$39.33$& $14.68$& $21.94$& $59.58$\\
Llama3\textsubscript{SB}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{SB-D}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{SB-FTD}&$-$& $-$& $-$& $-$\\

    \bottomrule % \thickhline

    \end{tabular}
    \caption{Baseline results on long document summarization.} %Results are reported as the average macro F1 over 5 random seeds.}
    \label{tab:baseline_results}
\end{table*}


==> tables/abstractive_results.tex <==

\begin{table*}[t]
    \centering
    
    \begin{tabular}{l c c | c c | c c | c c }
    \toprule %
    & \multicolumn{2}{ c |}{ SLT\textsuperscript{S} } & \multicolumn{2}{c|}{ LAS\textsuperscript{S} } & \multicolumn{2}{c |}{ SMH\textsuperscript{M} } & \multicolumn{2}{c |}{ SQB\textsuperscript{M} }\\
    \midrule
    Model & Rel & Con & Rel & Con & Rel & Con & Rel & Con\\

\midrule
Llama 3.2 1B &  $2.28$ & $1.63$ & $3.09$ & $\underline{2.88}$ & $3.52$ & $3.70$ & $2.90$ & $2.93$ \\
Fixed Gran. & $2.42$ & $1.49$ & $\underline{3.28}$ & $2.81$ & $3.09$ & $3.32$ & $\underline{3.28}$ & $\underline{3.36}$ \\
+ SUnsET & $\underline{2.60}$ & $\underline{2.23}$ & $2.99$ & $2.75$ & $3.82$ & $4.04$ & $3.17$ & $3.02$ \\
+ Shuffled & $2.57$ & $2.15$ & $3.06$ & $2.78$ & $\underline{3.83}$ & $\underline{4.35}$ & $3.18$ & $3.07$ \\\midrule
Llama 3.2 3B &  $\underline{3.66}$ & $\underline{3.52}$ & $\underline{4.26}$ & $\underline{4.49}$ & $4.47$ & $4.83$ & $3.99$ & $4.21$ \\
Fixed Gran. & $3.40$ & $3.11$ & $4.12$ & $4.34$ & $3.45$ & $3.53$ & $4.04$ & $\underline{4.28}$ \\
+ SUnsET & $3.49$ & $3.10$ & $4.13$ & $4.17$ & $4.73$ & $4.91$ & $4.26$ & $4.20$ \\
+ Shuffled & $3.16$ & $2.68$ & $4.17$ & $4.13$ & $\underline{4.88}$ & $\underline{4.95}$ & $\underline{4.36}$ & $4.20$ \\\midrule
Llama 3.1 8B &  $\underline{4.26}$ & $\underline{4.44}$ & $4.60$ & $\mathbf{\underline{4.81}}$ & $4.84$ & $4.92$ & $4.07$ & $4.24$ \\
Fixed Gran. & $4.23$ & $4.34$ & $4.59$ & $4.79$ & $4.43$ & $4.55$ & $4.52$ & $4.59$ \\
+ SUnsET & $4.23$ & $4.24$ & $4.65$ & $\mathbf{\underline{4.81}}$ & $4.89$ & $\mathbf{\underline{4.98}}$ & $4.58$ & $4.55$ \\
+ Shuffled & $4.08$ & $4.02$ & $\mathbf{\underline{4.66}}$ & $4.75$ & $\mathbf{\underline{4.92}}$ & $\mathbf{\underline{4.98}}$ & $\mathbf{\underline{4.68}}$ & $\mathbf{\underline{4.69}}$ \\\midrule
Mistral Nemo 2407 &  $4.15$ & $4.15$ & $3.52$ & $3.70$ & $4.05$ & $4.37$ & $3.09$ & $3.25$ \\
Fixed Gran. & $4.12$ & $4.26$ & $\underline{4.42}$ & $\underline{4.68}$ & $2.54$ & $2.62$ & $\underline{4.06}$ & $\underline{4.23}$ \\
+ SUnsET & $4.29$ & $4.31$ & $4.24$ & $4.39$ & $\underline{4.52}$ & $4.66$ & $3.65$ & $3.77$ \\
+ Shuffled & $\underline{4.41}$ & $\underline{4.38}$ & $4.35$ & $4.46$ & $4.50$ & $\underline{4.73}$ & $3.76$ & $3.86$ \\\midrule
Mixtral 8x7B &  $4.21$ & $4.47$ & $4.43$ & $4.73$ & $4.46$ & $4.67$ & $4.09$ & $4.27$ \\
Fixed Gran. & $4.46$ & $4.63$ & $4.46$ & $4.71$ & $3.93$ & $4.08$ & $4.19$ & $\underline{4.43}$ \\
+ SUnsET & $4.48$ & $4.64$ & $4.54$ & $4.79$ & $4.49$ & $4.74$ & $\underline{4.29}$ & $\underline{4.43}$ \\
+ Shuffled & $\mathbf{\underline{4.55}}$ & $\mathbf{\underline{4.67}}$ & $\underline{4.56}$ & $\mathbf{\underline{4.81}}$ & $\underline{4.55}$ & $\underline{4.78}$ & $4.20$ & $\underline{4.43}$ \\\midrule
\midrule GPT 4o Mini &  \textit{4.77} & \textit{4.85} & \textit{4.87} & \textit{4.93} & \textit{4.98} & \textit{5.00} & \textit{4.93} & \textit{4.94} \\
    \bottomrule %

    \end{tabular}
    \caption{Relevance and consistency of generated summaries. Relevance and consistency are measured using an autorater (DeepSeek-V3)~\cite{DBLP:conf/emnlp/LiuIXWXZ23} based on previously validated prompts~\cite{DBLP:journals/corr/abs-2410-23463}. 
    \textbf{Bold} indicates best overall performance, \underline{Underline} indicates best performance for individual models.
    \textsuperscript{S} indicates single document tasks, \textsuperscript{M} indicates multi-document. SQ is \sqa{}, LAS is \las{}, SMH is \smh{}, and SQB is \ops{}.}
    \label{tab:abstractive_results}
\end{table*}


==> tables/citation_results.tex <==

\begin{table*}[t]
    \centering

    \begin{tabular}{l c c | c c | c c | c c}
    \toprule %
    & \multicolumn{2}{ c |}{ SLT\textsuperscript{S} } & \multicolumn{2}{c|}{ LAS\textsuperscript{S} } & \multicolumn{2}{c |}{ SMH\textsuperscript{M} } & \multicolumn{2}{c}{ SQB\textsuperscript{M} }\\
    \midrule
    Model & Rel\textsubscript{F1} & Con\textsubscript{F1} & Rel\textsubscript{F1} & Con\textsubscript{F1} & Rel\textsubscript{F1} & Con\textsubscript{F1} & Rel\textsubscript{F1} & Con\textsubscript{F1}\\

\midrule
Llama 3.2 1B &  $0.14$ & $0.14$ & $1.22$ & $0.84$ & $0.36$ & $0.00$ & $0.11$ & $0.14$ \\
Fixed Gran. & $0.40$ & $0.13$ & $\underline{6.67}$ & $\underline{4.40}$ & $\underline{0.39}$ & $\underline{0.19}$ & $2.27$ & $\underline{1.35}$ \\
+ SUnsET & $1.18$ & $0.62$ & $5.43$ & $3.59$ & $0.00$ & $0.00$ & $\underline{3.13}$ & $1.26$ \\
+ Shuffled & $\underline{1.85}$ & $\underline{0.80}$ & $3.14$ & $3.04$ & $0.08$ & $0.00$ & $0.85$ & $0.72$ \\\midrule
Llama 3.2 3B &  $6.61$ & $3.86$ & $15.17$ & $13.29$ & $7.66$ & $6.52$ & $14.12$ & $10.54$ \\
Fixed Gran. & $21.71$ & $9.02$ & $\underline{45.80}$ & $\underline{41.44}$ & $1.37$ & $1.13$ & $\underline{27.77}$ & $\underline{23.49}$ \\
+ SUnsET & $\underline{25.36}$ & $\underline{14.76}$ & $33.42$ & $29.40$ & $\underline{32.21}$ & $\underline{29.59}$ & $13.76$ & $11.85$ \\
+ Shuffled & $15.14$ & $9.33$ & $19.45$ & $16.80$ & $26.78$ & $25.15$ & $17.45$ & $16.55$ \\\midrule
Llama 3.1 8B &  $11.66$ & $7.38$ & $28.89$ & $26.76$ & $32.07$ & $29.17$ & $20.73$ & $16.32$ \\
Fixed Gran. & $18.90$ & $11.32$ & $42.44$ & $38.86$ & $14.29$ & $14.23$ & $38.56$ & $37.64$ \\
+ SUnsET & $\underline{27.69}$ & $\underline{18.48}$ & $\mathbf{\underline{\mathbf{50.78}}}$ & $\mathbf{\underline{\mathbf{47.62}}}$ & $\mathbf{\underline{\mathbf{53.62}}}$ & $\mathbf{\underline{\mathbf{51.43}}}$ & $\mathbf{\underline{\mathbf{44.03}}}$ & $\underline{40.49}$ \\
+ Shuffled & $23.13$ & $16.12$ & $44.16$ & $41.18$ & $48.72$ & $46.50$ & $41.49$ & $39.59$ \\\midrule
Mistral Nemo 2407 &  $0.53$ & $0.23$ & $1.36$ & $1.29$ & $6.68$ & $6.68$ & $6.08$ & $5.54$ \\
Fixed Gran. & $6.61$ & $3.93$ & $13.36$ & $11.95$ & $3.71$ & $3.36$ & $15.05$ & $11.03$ \\
+ SUnsET & $\underline{21.71}$ & $\underline{13.99}$ & $\underline{23.38}$ & $\underline{23.09}$ & $\underline{20.73}$ & $\underline{19.71}$ & $\underline{22.00}$ & $\underline{20.61}$ \\
+ Shuffled & $17.67$ & $11.96$ & $22.85$ & $22.42$ & $19.82$ & $18.38$ & $16.87$ & $16.14$ \\\midrule
Mixtral 8x7B &  $17.83$ & $12.64$ & $34.27$ & $35.23$ & $33.40$ & $32.02$ & $17.30$ & $15.48$ \\
Fixed Gran. & $\mathbf{\underline{\mathbf{36.35}}}$ & $\mathbf{\underline{\mathbf{20.33}}}$ & $\underline{42.34}$ & $\underline{40.15}$ & $8.45$ & $7.46$ & $\underline{40.06}$ & $\mathbf{\underline{\mathbf{44.4}0}}$ \\
+ SUnsET & $22.60$ & $16.11$ & $35.81$ & $35.81$ & $42.91$ & $42.27$ & $28.61$ & $26.94$ \\
+ Shuffled & $23.79$ & $17.85$ & $37.21$ & $37.57$ & $\underline{43.89}$ & $\underline{42.98}$ & $32.25$ & $31.16$ \\\midrule
\midrule GPT 4o Mini &  \textit{37.39} & \textit{31.70} & \textit{61.17} & \textit{58.68} & \textit{63.61} & \textit{62.35} & \textit{33.71} & \textit{28.63} \\
    \bottomrule %

    \end{tabular}
    \caption{Relevance and consistency of evidence sentences with respect to their citances. Relevance and consistency are measured using an autorater (DeepSeek-V3)~\cite{DBLP:conf/emnlp/LiuIXWXZ23} based on previously validated prompts~\cite{DBLP:journals/corr/abs-2410-23463}. 
    We follow a similar setup to \cite{DBLP:conf/emnlp/LabanFXW24,openscholar} where we measure citation precision and recall in order to calculate an overall F1 score for both relevance and consistency. 
    \	extbf{Bold} indicates best overall performance, \underline{Underline} indicates best performance for individual models.
    \textsuperscript{S} indicates single document tasks, \textsuperscript{M} indicates multi-document. SQ is \sqa{}, LAS is \las{}, SMH is \smh{}, and SQB is \ops{}}
    \label{tab:retrieval_results}
\end{table*}


==> tables/citation_results_F1.tex <==

\begin{table*}[t]
    \centering

    \begin{tabular}{l c c | c c | c c | c c}
    \toprule %
    & \multicolumn{2}{ c |}{ SLT\textsuperscript{S} } & \multicolumn{2}{c|}{ LAS\textsuperscript{S} } & \multicolumn{2}{c |}{ SMH\textsuperscript{M} } & \multicolumn{2}{c}{ SQB\textsuperscript{M} }\\
    \midrule
    Model & Rel\textsubscript{F1} & Con\textsubscript{F1} & Rel\textsubscript{F1} & Con\textsubscript{F1} & Rel\textsubscript{F1} & Con\textsubscript{F1} & Rel\textsubscript{F1} & Con\textsubscript{F1}\\

\midrule
Llama 3.2 1B &  $0.14$ & $0.14$ & $1.22$ & $0.84$ & $0.36$ & $0.00$ & $0.11$ & $0.14$ \\
Fixed Gran. & $0.40$ & $0.13$ & $\underline{6.67}$ & $\underline{4.40}$ & $\underline{0.39}$ & $\underline{0.19}$ & $2.27$ & $\underline{1.35}$ \\
+ SUnsET & $1.18$ & $0.62$ & $5.43$ & $3.59$ & $0.00$ & $0.00$ & $\underline{3.13}$ & $1.26$ \\
+ Shuffled & $\underline{1.85}$ & $\underline{0.80}$ & $3.14$ & $3.04$ & $0.08$ & $0.00$ & $0.85$ & $0.72$ \\\midrule
Llama 3.2 3B &  $6.61$ & $3.86$ & $15.17$ & $13.29$ & $7.66$ & $6.52$ & $14.12$ & $10.54$ \\
Fixed Gran. & $21.71$ & $9.02$ & $\underline{45.80}$ & $\underline{41.44}$ & $1.37$ & $1.13$ & $\underline{27.77}$ & $\underline{23.49}$ \\
+ SUnsET & $\underline{25.36}$ & $\underline{14.76}$ & $33.42$ & $29.40$ & $\underline{32.21}$ & $\underline{29.59}$ & $13.76$ & $11.85$ \\
+ Shuffled & $15.14$ & $9.33$ & $19.45$ & $16.80$ & $26.78$ & $25.15$ & $17.45$ & $16.55$ \\\midrule
Llama 3.1 8B &  $11.66$ & $7.38$ & $28.89$ & $26.76$ & $32.07$ & $29.17$ & $20.73$ & $16.32$ \\
Fixed Gran. & $18.90$ & $11.32$ & $42.44$ & $38.86$ & $14.29$ & $14.23$ & $38.56$ & $37.64$ \\
+ SUnsET & $\underline{27.69}$ & $\underline{18.48}$ & $\mathbf{\underline{\mathbf{50.78}}}$ & $\mathbf{\underline{\mathbf{47.62}}}$ & $\mathbf{\underline{\mathbf{53.62}}}$ & $\mathbf{\underline{\mathbf{51.43}}}$ & $\mathbf{\underline{\mathbf{44.03}}}$ & $\underline{40.49}$ \\
+ Shuffled & $23.13$ & $16.12$ & $44.16$ & $41.18$ & $48.72$ & $46.50$ & $41.49$ & $39.59$ \\\midrule
Mistral Nemo 2407 &  $0.53$ & $0.23$ & $1.36$ & $1.29$ & $6.68$ & $6.68$ & $6.08$ & $5.54$ \\
Fixed Gran. & $6.61$ & $3.93$ & $13.36$ & $11.95$ & $3.71$ & $3.36$ & $15.05$ & $11.03$ \\
+ SUnsET & $\underline{21.71}$ & $\underline{13.99}$ & $\underline{23.38}$ & $\underline{23.09}$ & $\underline{20.73}$ & $\underline{19.71}$ & $\underline{22.00}$ & $\underline{20.61}$ \\
+ Shuffled & $17.67$ & $11.96$ & $22.85$ & $22.42$ & $19.82$ & $18.38$ & $16.87$ & $16.14$ \\\midrule
Mixtral 8x7B &  $17.83$ & $12.64$ & $34.27$ & $35.23$ & $33.40$ & $32.02$ & $17.30$ & $15.48$ \\
Fixed Gran. & $\mathbf{\underline{\mathbf{36.35}}}$ & $\mathbf{\underline{\mathbf{20.33}}}$ & $\underline{42.34}$ & $\underline{40.15}$ & $8.45$ & $7.46$ & $\underline{40.06}$ & $\mathbf{\underline{\mathbf{44.4}0}}$ \\
+ SUnsET & $22.60$ & $16.11$ & $35.81$ & $35.81$ & $42.91$ & $42.27$ & $28.61$ & $26.94$ \\
+ Shuffled & $23.79$ & $17.85$ & $37.21$ & $37.57$ & $\underline{43.89}$ & $\underline{42.98}$ & $32.25$ & $31.16$ \\\midrule
\midrule GPT 4o Mini &  \textit{37.39} & \textit{31.70} & \textit{61.17} & \textit{58.68} & \textit{63.61} & \textit{62.35} & \textit{33.71} & \textit{28.63} \\
    \bottomrule %

    \end{tabular}
    \caption{Relevance and consistency \textbf{F1} of evidence sentences with respect to their citances.
    We follow a similar setup to \cite{{DBLP:conf/emnlp/LabanFXW24,openscholar}} where we measure citation precision and recall in order to calculate an overall F1 score for both relevance and consistency.
    \textbf{Bold} indicates best overall performance, \underline{Underline} indicates best performance for individual models.
    \textsuperscript{S} indicates single document tasks, \textsuperscript{M} indicates multi-document. SQ is \sqa{}, LAS is \las{}, SMH is \smh{}, and SQB is \ops{}}
    \label{tab:retrieval_results_F1}
\end{table*}


==> tables/citation_results_precision.tex <==

\begin{table*}[t]
    \centering

    \begin{tabular}{l c c | c c | c c | c c}
    \toprule %
    & \multicolumn{2}{ c |}{ SLT\textsuperscript{S} } & \multicolumn{2}{c|}{ LAS\textsuperscript{S} } & \multicolumn{2}{c |}{ SMH\textsuperscript{M} } & \multicolumn{2}{c}{ SQB\textsuperscript{M} }\\
    \midrule
    Model & Rel\textsubscript{Prec} & Con\textsubscript{Prec} & Rel\textsubscript{Prec} & Con\textsubscript{Prec} & Rel\textsubscript{Prec} & Con\textsubscript{Prec} & Rel\textsubscript{Prec} & Con\textsubscript{Prec}\\

\midrule
Llama 3.2 1B &  $12.50$ & $12.50$ & $30.94$ & $20.51$ & $\underline{50.00}$ & $0.00$ & $37.50$ & $\underline{50.00}$ \\
Fixed Gran. & $19.86$ & $4.10$ & $39.22$ & $25.86$ & $25.94$ & $\underline{8.88}$ & $21.82$ & $11.47$ \\
+ SUnsET & $18.80$ & $10.61$ & $41.27$ & $32.05$ & $0.00$ & $0.00$ & $45.18$ & $24.08$ \\
+ Shuffled & $\underline{28.60}$ & $\underline{13.01}$ & $\underline{50.34}$ & $\underline{48.86}$ & $\underline{50.00}$ & $0.00$ & $\underline{62.38}$ & $48.20$ \\\midrule
Llama 3.2 3B &  $34.27$ & $20.34$ & $62.30$ & $55.77$ & $54.34$ & $44.53$ & $52.39$ & $39.86$ \\
Fixed Gran. & $34.84$ & $15.24$ & $62.02$ & $\underline{56.35}$ & $24.59$ & $24.91$ & $35.86$ & $29.97$ \\
+ SUnsET & $\underline{45.17}$ & $25.65$ & $61.16$ & $53.96$ & $64.75$ & $59.25$ & $52.91$ & $45.00$ \\
+ Shuffled & $44.28$ & $\underline{27.20}$ & $\underline{62.76}$ & $54.42$ & $\underline{65.76}$ & $\underline{62.84}$ & $\underline{60.98}$ & $\underline{56.37}$ \\\midrule
Llama 3.1 8B &  $42.69$ & $27.70$ & $67.18$ & $61.79$ & $62.72$ & $57.14$ & $49.95$ & $39.24$ \\
Fixed Gran. & $44.45$ & $26.84$ & $59.66$ & $54.80$ & $39.14$ & $39.00$ & $50.21$ & $49.70$ \\
+ SUnsET & $50.91$ & $33.71$ & $\underline{75.21}$ & $\underline{70.45}$ & $\mathbf{\underline{\mathbf{74.31}}}$ & $\underline{70.96}$ & $\underline{67.36}$ & $\underline{61.17}$ \\
+ Shuffled & $\underline{53.13}$ & $\underline{36.79}$ & $\mathbf{73.78}$ & $68.99$ & $70.55$ & $67.15$ & $64.70$ & $61.12$ \\\midrule
Mistral Nemo 2407 &  $31.67$ & $14.00$ & $60.27$ & $53.41$ & $\underline{\mathbf{73.78}}$ & $\mathbf{\underline{\mathbf{73.78}}}$ & $69.49$ & $61.38$ \\
Fixed Gran. & $32.44$ & $19.12$ & $60.28$ & $54.00$ & $29.59$ & $25.97$ & $37.86$ & $28.03$ \\
+ SUnsET & $\mathbf{\underline{\mathbf{57.34}}}$ & $36.90$ & $78.96$ & $\underline{78.69}$ & $73.62$ & $70.84$ & $\mathbf{\underline{\mathbf{71.44}}}$ & $\underline{66.50}$ \\
+ Shuffled & $56.07$ & $\underline{38.18}$ & $\underline{78.97}$ & $78.39$ & $70.58$ & $65.37$ & $64.97$ & $61.20$ \\\midrule
Mixtral 8x7B &  $47.82$ & $32.79$ & $81.58$ & $83.76$ & $68.54$ & $66.53$ & $53.67$ & $48.02$ \\
Fixed Gran. & $43.78$ & $24.11$ & $64.14$ & $61.01$ & $37.43$ & $29.62$ & $61.32$ & $\mathbf{\underline{\mathbf{67.63}}}$ \\
+ SUnsET & $50.74$ & $35.96$ & $82.94$ & $82.94$ & $69.77$ & $69.82$ & $60.82$ & $57.49$ \\
+ Shuffled & $\underline{52.52}$ & $\mathbf{\underline{\mathbf{38.71}}}$ & $\mathbf{\underline{\mathbf{84.19}}}$ & $\mathbf{\underline{\mathbf{85.29}}}$ & $\underline{73.80}$ & $\underline{73.33}$ & $\underline{61.94}$ & $59.22$ \\\midrule
\midrule GPT 4o Mini &  \textit{60.11} & \textit{52.11} & \textit{77.92} & \textit{74.76} & \textit{77.09} & \textit{75.57} & \textit{57.49} & \textit{49.18} \\
    \bottomrule %

    \end{tabular}
    \caption{Relevance and consistency \textbf{precision} of evidence sentences with respect to their citances.
    Precision measures the average citation quality within a given summary.
    \textbf{Bold} indicates best overall performance, \underline{Underline} indicates best performance for individual models.
    \textsuperscript{S} indicates single document tasks, \textsuperscript{M} indicates multi-document. SQ is \sqa{}, LAS is \las{}, SMH is \smh{}, and SQB is \ops{}}
    \label{tab:retrieval_results_precision}
\end{table*}


==> tables/citation_results_recall.tex <==

\begin{table*}[t]
    \centering

    \begin{tabular}{l c c | c c | c c | c c}
    \toprule %
    & \multicolumn{2}{ c |}{ SLT\textsuperscript{S} } & \multicolumn{2}{c|}{ LAS\textsuperscript{S} } & \multicolumn{2}{c |}{ SMH\textsuperscript{M} } & \multicolumn{2}{c}{ SQB\textsuperscript{M} }\\
    \midrule
    Model & Rel\textsubscript{Rec} & Con\textsubscript{Rec} & Rel\textsubscript{Rec} & Con\textsubscript{Rec} & Rel\textsubscript{Rec} & Con\textsubscript{Rec} & Rel\textsubscript{Rec} & Con\textsubscript{Rec}\\

\midrule
Llama 3.2 1B &  $0.10$ & $0.10$ & $0.94$ & $0.69$ & $0.27$ & $0.00$ & $0.06$ & $0.08$ \\
Fixed Gran. & $0.33$ & $0.12$ & $\underline{5.24}$ & $\underline{3.42}$ & $\underline{0.28}$ & $\underline{0.15}$ & $1.88$ & $\underline{1.14}$ \\
+ SUnsET & $0.82$ & $0.43$ & $4.06$ & $2.45$ & $0.00$ & $0.00$ & $\underline{2.40}$ & $0.93$ \\
+ Shuffled & $\underline{1.26}$ & $\underline{0.52}$ & $2.01$ & $1.94$ & $0.05$ & $0.00$ & $0.48$ & $0.41$ \\\midrule
Llama 3.2 3B &  $4.85$ & $2.82$ & $11.64$ & $10.13$ & $5.75$ & $4.90$ & $11.22$ & $8.36$ \\
Fixed Gran. & $18.13$ & $7.45$ & $\underline{39.63}$ & $\underline{35.85}$ & $0.93$ & $0.78$ & $\underline{24.02}$ & $\underline{20.37}$ \\
+ SUnsET & $\underline{20.14}$ & $\underline{11.86}$ & $26.95$ & $23.70$ & $\underline{26.68}$ & $\underline{24.54}$ & $10.18$ & $8.80$ \\
+ Shuffled & $11.09$ & $6.85$ & $14.56$ & $12.55$ & $22.24$ & $20.82$ & $11.53$ & $11.07$ \\\midrule
Llama 3.1 8B &  $8.90$ & $5.61$ & $22.41$ & $20.76$ & $25.52$ & $23.23$ & $16.68$ & $13.17$ \\
Fixed Gran. & $14.88$ & $8.98$ & $36.83$ & $33.73$ & $12.22$ & $12.19$ & $33.55$ & $\underline{32.60}$ \\
+ SUnsET & $\underline{21.32}$ & $\underline{14.28}$ & $\mathbf{\underline{\mathbf{41.31}}}$ & $\mathbf{\underline{\mathbf{38.72}}}$ & $\mathbf{\underline{\mathbf{47.39}}}$ & $\mathbf{\underline{\mathbf{45.45}}}$ & $\mathbf{\underline{\mathbf{35.28}}}$ & $32.47$ \\
+ Shuffled & $16.80$ & $11.70$ & $35.13$ & $32.78$ & $42.35$ & $40.44$ & $32.31$ & $30.86$ \\\midrule
Mistral Nemo 2407 &  $0.47$ & $0.20$ & $1.13$ & $1.08$ & $5.18$ & $5.17$ & $4.94$ & $4.54$ \\
Fixed Gran. & $5.39$ & $3.26$ & $10.40$ & $9.34$ & $2.64$ & $2.39$ & $12.04$ & $8.79$ \\
+ SUnsET & $\underline{17.48}$ & $\underline{11.30}$ & $\underline{19.93}$ & $\underline{19.66}$ & $\underline{16.63}$ & $\underline{15.80}$ & $\underline{17.68}$ & $\underline{16.59}$ \\
+ Shuffled & $13.81$ & $9.38$ & $19.59$ & $19.14$ & $16.17$ & $15.06$ & $13.54$ & $13.00$ \\\midrule
Mixtral 8x7B &  $15.47$ & $11.04$ & $29.99$ & $30.85$ & $29.87$ & $28.54$ & $13.92$ & $12.46$ \\
Fixed Gran. & $\mathbf{\underline{\mathbf{33.32}}}$ & $\mathbf{\underline{\mathbf{18.68}}}$ & $\underline{36.40}$ & $\underline{34.42}$ & $6.32$ & $5.75$ & $\underline{34.11}$ & $\mathbf{\underline{\mathbf{37.82}}}$ \\
+ SUnsET & $19.06$ & $13.64$ & $30.65$ & $30.68$ & $37.91$ & $37.31$ & $23.06$ & $21.80$ \\
+ Shuffled & $20.40$ & $15.40$ & $31.82$ & $32.08$ & $\underline{39.55}$ & $\underline{38.65}$ & $27.00$ & $26.22$ \\\midrule
\midrule GPT 4o Mini &  \textit{28.38} & \textit{23.86} & \textit{51.15} & \textit{49.07} & \textit{55.03} & \textit{53.93} & \textit{25.82} & \textit{21.99} \\
    \bottomrule %

    \end{tabular}
    \caption{Relevance and consistency \textbf{recall} of evidence sentences with respect to their citances.
    Recall measures citation quality and averages based on the total number of sentences in a summary. This penalizes models which produce fewer citations.
    \textbf{Bold} indicates best overall performance, \underline{Underline} indicates best performance for individual models.
    \textsuperscript{S} indicates single document tasks, \textsuperscript{M} indicates multi-document. SQ is \sqa{}, LAS is \las{}, SMH is \smh{}, and SQB is \ops{}}
    \label{tab:retrieval_results_recall}
\end{table*}


==> tables/evidence_hallucination.tex <==

\begin{table}[t]%
    \setlength{\tabcolsep}{3.5pt}
    \def\arraystretch{1.0}
    \centering
    \fontsize{8}{8}\selectfont
    \begin{tabular}{l c c c}
    \toprule %
    Model & Exact Match & 50\% Match & \# Evidence\\
\midrule
Llama 3.2 1B &  ~0.0 & 35.71 & ~~~~14 \\
+ \dataset{} & ~~\textbf{7.69} & \textbf{43.26} & ~~208\\
+ Shuffle & ~~5.15 & 22.68 & ~~~~97\\\midrule
Llama 3.2 3B &  25.57 & \textbf{90.11} & 1345\\
+ \dataset{} & \textbf{52.77} & 85.62 & 3720\\
+ Shuffle & 32.99 & 74.07 & 2337 \\\midrule
Llama 3.1 8B &  43.93 & 83.12 & 3412\\
+ \dataset{} & \textbf{78.36} & \textbf{97.21} & 4690\\
+ Shuffle & 54.53 & 88.51 & 4684 \\\midrule
Mistral Nemo 2407 &  ~~5.48 & 66.13 & ~~310\\
+ \dataset{} & \textbf{82.20} & \textbf{97.29} & 2107\\
+ Shuffle & 72.38 & 95.76 & 1959 \\\midrule
Mixtral 8x7B &  ~~5.79 & 91.25 & 3452\\
+ \dataset{} & \textbf{33.82} & 90.47 & 4208\\
+ Shuffle & 29.29 & \textbf{90.74} & 4288\\
\midrule
\midrule
GPT-4o-mini & \textit{11.06} & \textit{96.32} & \textit{8159}\\
    \bottomrule %

    \bottomrule %

    \end{tabular}
    \caption{
    Evidence copy rates. We measure exact string match (i.e. when the evidence sentence \textit{exactly} appears in the context) as well as 50\% overlap between the extracted evidence and the longest common substring.} %
    \vspace{-7pt}
    \label{tab:hallucination_results}
\end{table}


==> tables/models_description.tex <==
\begin{table}[t]
    \def\arraystretch{1.1}
    \centering
    \scriptsize
    \begin{tabular}{l|c}
    \toprule
    Model & Huggingface Identifier \\
    \midrule
       Llama 3.2 1B  & \texttt{meta-llama/Llama-3.2-1B-Instruct} \\
        Llama 3.2 3B & \texttt{meta-llama/Llama-3.2-3B-Instruct} \\
         Llama 3.1 8B & \texttt{meta-llama/Meta-Llama-3.1-8B-Instruct} \\ 
          Mistral Nemo 2407 & \texttt{mistralai/Mistral-Nemo-Instruct-2407} \\
          Mixtral 8x7B & \texttt{mistralai/Mixtral-8x7B-Instruct-v0.1} \\
          \bottomrule
    \end{tabular}
    \caption{Huggingface identifiers for models used in our experiments.}
    \label{tab:models_description}
\end{table}


==> tables/synthetic_data.tex <==

\begin{table}[t]%
    \setlength{\tabcolsep}{2pt}
    \def\arraystretch{1.1}
    \centering
    \fontsize{7.8}{7.8}\selectfont
    \rowcolors{2}{gray!15}{white}
    \begin{tabular}{r c c c | c c c | c c c}
    \toprule %
    & \multicolumn{3}{ c |}{ \dataset{} } & \multicolumn{3}{c|}{ Non-Pipelined } & \multicolumn{3}{c}{ Title + Doc } \\
    \midrule
    
    \cellcolor{black!75}\color{white}Metric & Q & S & D  & Q & S & D & Q & S & D \\
    \cellcolor{black!75}\color{white}TTR & \textbf{0.75} & \textbf{0.84} & \textbf{0.82} &  0.67 & 0.80 & 0.35 & 0.63 & 0.78 & 0.35 \\
    \cellcolor{black!75}\color{white}Cos & \textbf{0.81} & \textbf{0.73} & \textbf{0.68} &  0.73 & 0.72 & 0.04 & 0.66 & 0.61 & 0.04 \\
    \cellcolor{black!75}\color{white}Len & \textbf{13.45} & \textbf{226.5} & \textbf{3767.4} & 9.85 & 23.79 & 474.8 & 10.21 & 24.45 & 433.8 \\
    
    

    \bottomrule %

    \end{tabular}
    \caption{Statistics and diversity metrics of synthetic data. Metrics are average type-token ratio (TTR) \citet{DBLP:journals/corr/abs-2307-04626}, embedding cosine distance (Cos), and average word length (Len). Columns differentiate between (Q)uestion, (S)ummary and (D)ocument metrics in each dataset. \textbf{Bold} is highest diversity across datasets.} %
    \label{tab:synthetic_stats}
\end{table}


==> tables/table1.tex <==

\begin{table*}%
    \def\arraystretch{1.2}
    \centering
    \scriptsize
    \begin{tabular}{l c c c c}
    \toprule %
    Method & R1 & R2 & RL & BERTScore\\

\midrule
\multicolumn{5}{c}{ACLSum \cite{DBLP:journals/corr/abs-2403-05303}}\\
\midrule
Llama2\textsubscript{ZS} \cite{DBLP:journals/corr/abs-2403-05303} & $26.17$&$9.43$&$18.91$&$64.00$ \\
Mistral\textsubscript{ZS}&$34.40$& $12.07$& $25.13$& $66.97$\\
Mistral\textsubscript{WiM}&$-$& $-$& $-$& $-$\\
Mistral\textsubscript{CB}&$33.75$& $11.73$& $24.69$& $66.59$\\
Mistral\textsubscript{CB-D}&$\mathbf{35.10}$& $12.44$& $25.12$& $\mathbf{67.63}$\\
Mistral\textsubscript{CB-FTD}&$34.67$& $12.29$& $\mathbf{25.58}$& $67.46$\\
Mistral\textsubscript{SB}&$33.41$& $11.13$& $24.24$& $66.45$\\
Mistral\textsubscript{SB-D}&$34.36$& $12.28$& $25.13$& $66.95$\\
Mistral\textsubscript{SB-FTD}&$33.95$& $11.77$& $24.71$& $66.96$\\
Llama3\textsubscript{ZS}&$33.85$& $12.61$& $24.74$& $67.09$\\
Llama3\textsubscript{WiM}&$32.70$& $12.91$& $24.79$& $66.18$\\
Llama3\textsubscript{CB}&$32.42$& $11.45$& $23.70$& $66.34$\\
Llama3\textsubscript{CB-D}&$34.03$& $12.28$& $24.87$& $67.23$\\
Llama3\textsubscript{CB-FTD}&$34.51$& $\mathbf{13.00}$& $25.04$& $67.33$\\
Llama3\textsubscript{SB}&$31.95$& $11.27$& $23.49$& $66.15$\\
Llama3\textsubscript{SB-D}&$33.54$& $12.61$& $24.71$& $66.84$\\
Llama3\textsubscript{SB-FTD}&$33.41$& $12.44$& $24.68$& $67.00$\\
\midrule
\multicolumn{5}{c}{SQuALITY \cite{DBLP:conf/emnlp/WangPCPB22}}\\
\midrule
BART+DPR \cite{DBLP:conf/emnlp/WangPCPB22} & $41.50$&$11.40$&$21.00$&$85.50$ \\
Mistral\textsubscript{ZS}&$\mathbf{37.75}$& $9.22$& $\mathbf{19.89}$& $\mathbf{61.48}$\\
Mistral\textsubscript{WiM}&$36.50$& $\mathbf{9.36}$& $19.34$& $59.01$\\
Mistral\textsubscript{CB}&$37.29$& $8.95$& $19.35$& $60.34$\\
Mistral\textsubscript{CB-D}&$36.92$& $8.54$& $19.29$& $60.73$\\
Mistral\textsubscript{CB-FTD}&$36.87$& $8.96$& $19.18$& $60.26$\\
Mistral\textsubscript{SB}&$-$& $-$& $-$& $-$\\
Mistral\textsubscript{SB-D}&$-$& $-$& $-$& $-$\\
Mistral\textsubscript{SB-FTD}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{ZS}&$34.18$& $8.26$& $18.11$& $55.47$\\
Llama3\textsubscript{WiM}&$33.34$& $8.78$& $18.12$& $57.25$\\
Llama3\textsubscript{CB}&$34.60$& $8.37$& $18.31$& $56.27$\\
Llama3\textsubscript{CB-D}&$34.57$& $8.20$& $18.28$& $56.07$\\
Llama3\textsubscript{CB-FTD}&$34.30$& $8.10$& $18.22$& $56.06$\\
Llama3\textsubscript{SB}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{SB-D}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{SB-FTD}&$-$& $-$& $-$& $-$\\
\midrule
\multicolumn{5}{c}{LexAbSumm \cite{DBLP:conf/coling/SantoshAG24}}\\
\midrule
Unlimiformer-BART \cite{DBLP:conf/coling/SantoshAG24} & $50.62$&$30.28$&$35.55$&$88.86$ \\
Mistral\textsubscript{ZS}&$36.97$& $14.54$& $20.07$& $59.64$\\
Mistral\textsubscript{WiM}&$34.91$& $13.26$& $19.26$& $57.97$\\
Mistral\textsubscript{CB}&$37.00$& $13.85$& $20.22$& $59.41$\\
Mistral\textsubscript{CB-D}&$37.80$& $14.83$& $20.57$& $59.93$\\
Mistral\textsubscript{CB-FTD}&$38.41$& $\mathbf{15.26}$& $20.79$& $\mathbf{60.36}$\\
Mistral\textsubscript{SB}&$-$& $-$& $-$& $-$\\
Mistral\textsubscript{SB-D}&$-$& $-$& $-$& $-$\\
Mistral\textsubscript{SB-FTD}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{ZS}&$\mathbf{39.47}$& $15.06$& $\mathbf{22.28}$& $59.43$\\
Llama3\textsubscript{WiM}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{CB}&$38.44$& $13.86$& $21.62$& $59.08$\\
Llama3\textsubscript{CB-D}&$38.77$& $14.64$& $21.81$& $59.33$\\
Llama3\textsubscript{CB-FTD}&$39.33$& $14.68$& $21.94$& $59.58$\\
Llama3\textsubscript{SB}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{SB-D}&$-$& $-$& $-$& $-$\\
Llama3\textsubscript{SB-FTD}&$-$& $-$& $-$& $-$\\

    \bottomrule %

    \end{tabular}
    \caption{Baseline results on long document summarization.} %
    \label{tab:baseline_results}
\end{table*}


==> tables/topic_diversity.tex <==

\begin{table}[t]%
    \setlength{\tabcolsep}{2pt}
    \def\arraystretch{1.1}
    \centering
    \fontsize{7.8}{7.8}\selectfont
    \begin{tabular}{r c}
    \toprule %
    Dataset & Topic Diversity \\
    \midrule
    
    Non-Pipelined & \cellcolor{blue!20}0.506 \\
    Title + Doc & 0.356 \\
    \sqa{} (human, stories)& \cellcolor{blue!45}0.705 \\
   \las{} (human, legal text) & \cellcolor{blue!40}0.673 \\
    \ops{} (human, scientific docs) & \cellcolor{blue!44}0.695 \\
    \textbf{\dataset{}} & \cellcolor{blue!41}0.679 \\
    
    

    \bottomrule %

    \end{tabular}
    \caption{Topic diversity scores using the approach from \citet{DBLP:conf/eacl/TerragniFGTC21}. Shading indicates magnitude of diversity score.} %
    \label{tab:topic_diversity}
\end{table}

